Abductive World Modeling via Causal Representation Learning

The central challenge of world modeling is to learn representations that capture how the world evolves. However, existing world models predominantly represent future states without explicitly capturing the latent causes underlying their evolution, limiting their ability to reason about why and how the world changes. To address this limitation, we propose Abductive World Modeling (AWM), a framework that learns structured causal representations by abductively inferring latent causes from predicted futures. Specifically, we realize AWM through the Hierarchical Abductive State Pyramid (HASP), which organizes the inferred world state into three complementary components - Entity, Dynamic, and Relation - capturing what exists, how it changes, and how entities interact, respectively. By jointly reasoning over the current observation and its predicted future, HASP abductively infers these latent factors and integrates them into a structured state representation for downstream reasoning. To the best of our knowledge, AWM is the first framework to introduce abductive state inference into latent-space world modeling for learning structured representations of world dynamics. Experiments across physical prediction, causal reasoning, and action understanding demonstrate the effectiveness of our approach. Compared with V-JEPA, a state-of-the-art latent-space world model, AWM improves physical prediction AUROC by 10.7%, causal reasoning accuracy by 16.8%, and action Top-1 accuracy by 68.0%.

==> Table/clevrer_future_events.tex <==
\begin{table}[t]
\centering
\caption{Predicted-future evidence mainly improves interaction-time reasoning.}
\label{tab:clevrer-future-events}
\small
\renewcommand{\arraystretch}{1.05}
\begin{tabularx}{0.70\linewidth}{@{}Lcc@{}}
\toprule\toprule
\textbf{Metric} & \textbf{Context} & \textbf{Context + Future} \\
\midrule
Contact AUROC & 96.2 & 97.2 \\
Contact AP & 20.4 & 26.5 \\
First-contact accuracy & 94.0 & 94.5 \\
Collision-pair first-contact & 17.1 & 25.4 \\
\bottomrule\bottomrule
\end{tabularx}
\end{table}


==> Table/clevrer_future_predictability.tex <==
\begin{table*}[t]
\centering
\caption{CLEVRER future-state predictability with and without predicted-future
evidence.  The current-only branch receives context latent only.}
\label{tab:clevrer-future-predictability}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Metric} & \textbf{Context only} & \makecell{\textbf{Context +}\\\textbf{predicted future}} & \textbf{Difference} \\
\midrule
Presence F1 & 93.0\% & 93.1\% & +0.1\pp \\
Color accuracy & 83.0\% & 83.5\% & +0.5\pp \\
Material accuracy & 93.3\% & 91.0\% & -2.3\pp \\
Shape accuracy & 91.5\% & 93.5\% & +2.0\pp \\
Center MAE & 0.0569 & 0.0612 & +0.0043 \\
Pair-distance MAE & 0.0838 & 0.0879 & +0.0041 \\
Contact AUROC & 96.2\% & \best{97.2\%} & +1.0\pp \\
First-contact accuracy & 94.0\% & 94.5\% & +0.5\pp \\
Collision-pair first-contact accuracy & 17.1\% & \best{25.4\%} & +8.3\pp \\
No-contact pair accuracy & 99.6\% & 99.4\% & -0.2\pp \\
\bottomrule
\end{tabular}
\end{table*}


==> Table/clevrer_relation_interaction.tex <==
\begin{table}[t]
\centering
\caption{Contribution of different state components to interaction prediction on CLEVRER. Higher Contact AUROC is better, while lower TTC MAE is better.}
\label{tab:relation-component-control}
\small
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Feature} & \textbf{Contact AUROC} & \textbf{TTC MAE} \\
\midrule
Entity-only   & 0.9295 & 0.1411 \\
Dynamic-only  & 0.9499 & 0.1138 \\
Relation-only & 0.9673 & 0.1054 \\
Full          & \textbf{0.9680} & \textbf{0.1049} \\
\bottomrule
\end{tabular}
\end{table}

==> Table/cross_task_reuse.tex <==
\begin{table}[t]
\centering
\caption{Cross-task reuse of individual state factors on EK100.}
\label{tab:layer-transfer}
\small
\renewcommand{\arraystretch}{1.05}
\begin{tabularx}{0.70\linewidth}{@{}Lcc@{}}
\toprule\toprule
\textbf{State level} & \textbf{Verb Top-1} & \textbf{Noun Top-1} \\
\midrule
Entity & 50.43\% & 31.61\% \\
Dynamic & \best{56.98\%} & \best{33.03\%} \\
Relation & 30.99\% & 16.73\% \\
\bottomrule\bottomrule
\end{tabularx}
\end{table}


==> Table/dynamic_information.tex <==
\begin{table}[t]
\centering
\caption{Dynamic-state readability at the slot--time level.}
\label{tab:dynamic-information}
\small
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Target} & \textbf{Metric} & \textbf{Score} \\
\midrule
Speed & $R^2$ & 0.7198 \\
Velocity & $R^2$ & 0.3805 \\
\bottomrule
\end{tabular}
\end{table}


==> Table/entity_information.tex <==
\begin{table}[t]
\centering
\caption{Entity-state readability at the slot level.}
\label{tab:entity-information}
\small
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Target} & \textbf{Metric} & \textbf{Score} \\
\midrule
Presence & AUROC & 0.9634 \\
Extent & $R^2$ & 0.5316 \\
\bottomrule
\end{tabular}
\end{table}


==> Table/future_evidence_pair.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.03}
\begin{minipage}[t]{0.48\linewidth}
\vspace{0pt}
\refstepcounter{table}\label{tab:physion-future-semantics}
\centering
\parbox[t][2.6em][t]{\linewidth}{\centering\textbf{Table~\thetable.} Effect of predicted-future evidence on present-state decoding.}\par\smallskip
\begin{tabularx}{\linewidth}{@{}Lcc@{}}
\toprule\toprule
\textbf{Target} & \textbf{Context} & \textbf{Context + Future} \\
\midrule
Presence F1 & 99.58 & 99.77 \\
Target accuracy & 94.02 & 95.79 \\
Object type accuracy & 91.18 & 92.86 \\
\bottomrule\bottomrule
\end{tabularx}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\linewidth}
\vspace{0pt}
\refstepcounter{table}\label{tab:clevrer-future-events}
\centering
\parbox[t][2.6em][t]{\linewidth}{\centering\textbf{Table~\thetable.} Predicted-future evidence mainly improves interaction-time reasoning.}\par\smallskip
\begin{tabularx}{\linewidth}{@{}Lcc@{}}
\toprule\toprule
\textbf{Metric} & \textbf{Context} & \textbf{Context + Future} \\
\midrule
Contact AUROC & 96.2 & 97.2 \\
Contact AP & 20.4 & 26.5 \\
First-contact accuracy & 94.0 & 94.5 \\
Collision-pair first-contact & 17.1 & 25.4 \\
\bottomrule\bottomrule
\end{tabularx}
\end{minipage}
\end{table}


==> Table/granularity_specificity.tex <==
\begin{table*}[t]
\centering
\caption{Granularity and attribution specificity.  Native units are compared with
pooled and alignment-destroyed controls under matched-capacity probes.}
\label{tab:granularity-specificity}
\small
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Representation} & \textbf{Entity target} & \textbf{Dynamic target} & \textbf{Relation target} \\
\midrule
Native structured unit & \missing & \missing & \missing \\
Global pooled state & \missing & \missing & \missing \\
Shuffled slot/pair/time & \missing & \missing & \missing \\
\bottomrule
\end{tabular}
\end{table*}


==> Table/i_input_temporal_intervention.tex <==
\begin{table}[t]
\centering
\caption{
Temporal-static latent intervention on Physion++.
\textit{ASM} uses the original context and future features.
\textit{ASM w/o Temporal} temporally averages and repeats these features at each time step, removing temporal variation while keeping the model and readouts frozen.
}
\label{tab:input-temporal-intervention}
\small
\renewcommand{\arraystretch}{1.03}

\begin{tabularx}{\linewidth}{
@{}
>{\raggedright\arraybackslash}X
>{\centering\arraybackslash}X
>{\centering\arraybackslash}X
>{\centering\arraybackslash}X
@{}
}
\toprule\toprule
\textbf{Condition}
& \textbf{Speed MAE} ($\downarrow$)
& \textbf{Contact AUROC} ($\uparrow$)
& \textbf{OCP AUROC} ($\uparrow$) \\
\midrule

\textbf{ASM}
& \textbf{0.0670}
& \textbf{0.9837}
& \textbf{0.7907} \\

w/o Temporal
& 0.1120
& 0.9485
& 0.5646 \\

\bottomrule
\end{tabularx}
\end{table}


==> Table/i_main_results.tex <==
\begin{table}[t]
\centering
\caption{Main comparison across datasets. All entries are percentage values reported without the percent sign, and the best value in each metric column is boldfaced. ``Bal.~Acc.'' and ``Acc.'' denote balanced accuracy and accuracy, respectively, while EK100 results are reported as Top-1/Top-5. Orca and VideoMAE~v2 are marked as ``\textemdash'' on CLEVRER because their released models do not provide the predictive module required by the CLEVRER evaluation pipeline.}
\label{tab:main}
\scriptsize
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{0.92}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lccc cc ccc@{}}
\toprule\toprule
 & \multicolumn{3}{c}{\textbf{Physion++}} & \multicolumn{2}{c}{\textbf{CLEVRER}} & \multicolumn{3}{c}{\textbf{EK100 (T1/T5)}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-6}\cmidrule(lr){7-9}
\textbf{Method} & \textbf{AUROC} & \textbf{Bal.~Acc.} & \textbf{Acc.} & \textbf{Option Acc.} & \textbf{Question Acc.} & \textbf{Verb} & \textbf{Noun} & \textbf{Action} \\
\midrule
\vjepa{} & $65.20$ & $61.57$ & $61.60$ & $65.46$ & $42.20$ & $55.74/86.81$ & $34.65/62.67$ & $25.67/46.94$ \\
Orca & $59.15$ & $55.94$ & $56.64$ & \textemdash & \textemdash & $33.75/74.39$ & $21.54/45.36$ & $13.08/30.46$ \\
VideoMAE~v2 & $67.61$ & $62.60$ & $62.86$ & \textemdash & \textemdash & $59.54/82.57$ & $46.37/68.79$ & $35.96/54.57$ \\
\asm{} (Ours) & \best{72.19} & \best{66.17} & \best{65.63} & \best{70.89} & \best{49.31} & \best{69.05/91.27} & \best{47.59/75.05} & \best{43.12/67.34} \\
\bottomrule
\end{tabular}
}
\end{table}


==> Table/i_native_factor_information.tex <==
\begin{table}[t]
\centering
\caption{
Native factor readability on Physion++.
}
\label{tab:native-factor-information}

\scriptsize
\renewcommand{\arraystretch}{1.06}
\setlength{\tabcolsep}{3.5pt}

\begin{tabular*}{\linewidth}{
    @{\extracolsep{\fill}}
    l
    l
    c
    c
}
\toprule\toprule
\textbf{State}
& \textbf{Factor}
& \textbf{Metric}
& \textbf{Score} \\
\midrule

Entity
& Presence
& AUROC
& 0.9634 \\

& Spatial extent
& $R^2$
& 0.5316 \\

\addlinespace[1.5pt]

Dynamic
& Speed
& $R^2$
& 0.7198 \\

& Signed velocity
& $R^2$
& 0.3805 \\

\addlinespace[1.5pt]

Relation
& Contact
& AUROC
& 0.9789 \\

& Pairwise distance
& $R^2$
& 0.5815 \\

& Time-to-contact
& $R^2$
& 0.5542 \\

\bottomrule
\end{tabular*}

\end{table}


==> Table/i_parameter_setting.tex <==
\begin{table*}[ht]
    \centering
    \caption{
    \textbf{Main configuration and hyperparameter settings of ASM.}
    We report the predictive backbone, evaluation configuration, and computational setup used in our experiments.
    }
    \label{tab:parameter_setting}
    \resizebox{0.68\textwidth}{!}{
    \begin{tabular}{lc}
        \toprule\toprule
        \textbf{Parameter} & \textbf{Value} \\
        \midrule

        \multicolumn{2}{c}{\textbf{Predictive Backbone}} \\
        \midrule
        Backbone & V-JEPA 2 ViT-H \\
        Observed frames & 16 \\
        Predicted future frames & 16 \\
        Patch size & 16 \\
        Tubelet size & 2 \\
        Predictor depth & 12 \\
        Predictor embedding dimension & 384 \\
        Predictor attention heads & 12 \\

        \midrule
        \multicolumn{2}{c}{\textbf{Evaluation Configuration}} \\
        \midrule
        Visual encoder & Frozen \\
        Latent predictor & Frozen \\
        HASP state extractor & Frozen \\
        Trainable modules & Factor probes / task readouts \\
        Readout optimizer & AdamW \\
        Precision & BF16 \\
        Random seed & 239 \\

        \bottomrule
    \end{tabular}
    }
\end{table*}


==> Table/i_physion_confusion_intervention.tex <==
\begin{table}[t]
\centering
\caption{Physion++ OCP confusion counts under probe interventions.}
\label{tab:physion-confusion-intervention}
\scriptsize
\renewcommand{\arraystretch}{1.03}
\begin{tabularx}{0.70\linewidth}{@{}Lrrrr@{}}
\toprule\toprule
\textbf{Condition} & \textbf{TP} & \textbf{TN} & \textbf{FP} & \textbf{FN} \\
\midrule
Visual-only & 237 & 292 & 129 & 142 \\
Visual + ShallowProbe & 277 & 297 & 124 & 102 \\
Target mask & 325 & 181 & 240 & 54 \\
Irrelevant mask & 262 & 305 & 116 & 117 \\
Random slot & 279 & 294 & 127 & 100 \\
\bottomrule
\end{tabularx}
\end{table}


==> Table/i_physion_logit_intervention.tex <==
\begin{table}[t]
\centering
\caption{Paired OCP-logit changes under probe-level interventions.}
\label{tab:physion-logit-intervention}
\scriptsize
\renewcommand{\arraystretch}{1.03}
\begin{tabularx}{0.70\linewidth}{@{}Lcc@{}}
\toprule\toprule
\textbf{Condition} & \textbf{Mean change} & \textbf{Mean absolute change} \\
\midrule
Target mask & +0.49195 & 0.67680 \\
Irrelevant mask & -0.08051 & 0.17355 \\
Random slot & +0.02437 & 0.08895 \\
\bottomrule\bottomrule
\end{tabularx}
\end{table}


==> Table/i_physion_slot_diagnostics.tex <==
\begin{table}[t]
\centering
\caption{Additional diagnostics of the Physion++ Entity slots.}
\label{tab:physion-slot-diagnostics}
\scriptsize
\renewcommand{\arraystretch}{1.03}
\begin{tabularx}{0.70\linewidth}{@{}Lc@{}}
\toprule\toprule
\textbf{Diagnostic} & \textbf{Value} \\
\midrule
Presence F1 & 99.77 \\
Slot occupancy & 64.52 \\
Identity consistency & 70.29 \\
ID switch rate & 4.05 \\
Target-object accuracy & 95.79 \\
Object-type accuracy & 92.86 \\
Color RGB MAE & 0.2244 \\
Center MAE & 0.0454 \\
Geometry MAE & 0.0285 \\
Velocity MAE & 0.00629 \\
\bottomrule
\end{tabularx}
\end{table}


==> Table/i_query_intervention.tex <==
\begin{table}[t]
\centering
\caption{
Relevant-object intervention on CLEVRER predictive queries.
\textit{ASM} uses all Entity evidence;
\textit{ASM w/o Relevant Object} removes the object referred to by the query;
and \textit{ASM w/o Irrelevant Object} removes an object unrelated to the query.
}
\label{tab:query-intervention}
\small
\renewcommand{\arraystretch}{1.03}

\begin{tabularx}{0.78\linewidth}{@{}Lcccc@{}}
\toprule\toprule
\textbf{Condition}
& \makecell{\textbf{Question}\\\textbf{Correct}}
& \makecell{\textbf{Question}\\\textbf{Acc.} $\uparrow$}
& \makecell{\textbf{Option}\\\textbf{Correct}}
& \makecell{\textbf{Option}\\\textbf{Acc.} $\uparrow$} \\
\midrule
\textbf{ASM}
& 1,785/3,557
& \textbf{50.18\%}
& 5,099/7,114
& \textbf{71.68\%} \\

ASM w/o Relevant Object
& 1,546/3,557
& 43.46\%
& 4,752/7,114
& 66.80\% \\

ASM w/o Irrelevant Object
& 1,684/3,557
& 47.34\%
& 4,948/7,114
& 69.55\% \\
\bottomrule
\end{tabularx}
\end{table}


==> Table/i_relation_selective_intervention.tex <==
\begin{table}[t]
\centering
\caption{
Relation-pair intervention on CLEVRER.
\textit{ASM} uses all Relation pairs;
\textit{ASM w/o Contact Pair} removes the target contact pair;
and \textit{ASM w/o Non-contact Pair} removes an unrelated pair.
We report geometric and interaction prediction performance.
}
\label{tab:relation-selective-intervention}
\small
\renewcommand{\arraystretch}{1.05}

\begin{tabularx}{\linewidth}{
@{}
>{\raggedright\arraybackslash}X
>{\centering\arraybackslash}X
>{\centering\arraybackslash}X
>{\centering\arraybackslash}X
@{}
}
\toprule\toprule
\textbf{Condition}
& \textbf{Pair-dist. MAE} ($\downarrow$)
& \textbf{TTC MAE} ($\downarrow$)
& \textbf{Contact AUROC} ($\uparrow$) \\
\midrule

\textbf{ASM}
& \textbf{0.0196}
& \textbf{0.1306}
& \textbf{0.9633} \\

w/o Contact Pair
& 0.0225
& 0.1376
& 0.9488 \\

w/o Non-contact Pair
& 0.0208
& 0.1349
& 0.9518 \\

\bottomrule
\end{tabularx}
\end{table}


==> Table/input_evidence_intervention.tex <==
\begin{table*}[t]
\centering
\caption{Input-evidence interventions with frozen readouts.  Higher AUROC and lower
MAE are better.}
\label{tab:physion-input-intervention}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{\textwidth}{@{}lYYYYY@{}}
\toprule
 & \multicolumn{2}{c}{\textbf{Factor readout}} & \multicolumn{2}{c}{\textbf{Interaction}} & \textbf{Task} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
\textbf{Condition} & \makecell{Entity extent\\MAE} & \makecell{Dynamic speed\\MAE} & \makecell{Contact\\AUROC} & \makecell{TTC\\MAE} & \makecell{OCP\\AUROC} \\
\midrule
Cached baseline & 0.0292 & 0.0670 & 0.9837 & 0.1262 & 0.7907 \\
50\% object-guided mask & 0.0328 & 0.0739 & 0.9808 & 0.1307 & 0.7150 \\
50\% random mask & 0.0304 & 0.0692 & 0.9837 & 0.1278 & 0.7757 \\
Temporal static & 0.0580 & 0.1120 & 0.9485 & 0.2665 & 0.5646 \\
\bottomrule
\end{tabularx}
\end{table*}


==> Table/input_object_intervention.tex <==
\begin{table}[t]
\centering
\caption{
Entity intervention on Physion++ OCP prediction.
\textit{Full} uses all Entity slots;
\textit{Target mask} removes the slot corresponding to the target object;
and \textit{Irrelevant mask} removes a slot corresponding to a non-target object.
}
\label{tab:input-object-intervention}
\small
\renewcommand{\arraystretch}{1.03}

\begin{tabularx}{0.70\linewidth}{@{}Lccc@{}}
\toprule
\textbf{Condition} & \textbf{Accuracy} & \textbf{Bal. Acc.} & \textbf{AUROC} \\
\midrule
Full            & \textbf{0.7175} & \textbf{0.7182} & \textbf{0.7962} \\
Target mask     & 0.6325          & 0.6437          & 0.7391          \\
Irrelevant mask & 0.7088          & 0.7079          & 0.7834          \\
\bottomrule
\end{tabularx}
\end{table}


==> Table/native_factor_information.tex <==
\begin{table}[t]
\centering
\caption{
Native-factor readability of HASP states on Physion++.
Entity, Dynamic, and Relation are probed for object, motion,
and pairwise interaction factors, respectively.
Higher scores indicate better factor readability.
}
\label{tab:native-factor-information}

\small
\renewcommand{\arraystretch}{1.08}

\begin{tabular*}{0.78\linewidth}{
    @{\extracolsep{\fill}}
    l
    l
    c
    c
}
\toprule\toprule
\textbf{State}
& \textbf{Native Factor}
& \textbf{Probe Metric}
& \textbf{Score} ($\uparrow$) \\
\midrule

Entity
& Presence
& AUROC
& 0.9634 \\

& Spatial extent
& $R^2$
& 0.5316 \\

\addlinespace[2pt]

Dynamic
& Speed
& $R^2$
& 0.7198 \\

& Signed velocity
& $R^2$
& 0.3805 \\

\addlinespace[2pt]

Relation
& Contact
& AUROC
& 0.9789 \\

& Pairwise distance
& $R^2$
& 0.5815 \\

& Time-to-contact
& $R^2$
& 0.5542 \\

\bottomrule
\end{tabular*}

\end{table}

==> Table/native_factors.tex <==
\begin{table*}[t]
\centering
\caption{Native-factor probes on the physical validation set.  Higher $R^2$/AUROC
and lower MAE are better.}
\label{tab:native-factors}
\small
\setlength{\tabcolsep}{6.5pt}
\begin{tabular}{@{}llccc@{}}
\toprule
\textbf{State} & \textbf{Granularity} & \textbf{Target} & \textbf{MAE} & \makecell{\textbf{$R^2$ /}\\\textbf{AUROC}} \\
\midrule
Entity & slot & presence & \missing & 0.9634 AUROC \\
Entity & slot & extent & 0.0531 & 0.5316 \\
Dynamic & time & speed & 0.0760 & 0.7198 \\
Dynamic & time & velocity & 0.0432 & 0.3805 \\
Relation & pair & distance & 0.0369 & 0.5425 \\
Relation & pair & contact & \missing & 0.9847 AUROC \\
Relation & pair & time-to-contact & 0.0487 & 0.5542 \\
Relation & pair--time & distance & 0.0361 & 0.5815 \\
Relation & pair--time & contact & \missing & 0.9789 AUROC \\
\bottomrule
\end{tabular}
\end{table*}


==> Table/physion_future_input.tex <==
\begin{table*}[t]
\centering
\caption{Physical structured-probe diagnostics with and without predicted-future input
(4,129 matched objects).}
\label{tab:physion-full-current}
\small
\setlength{\tabcolsep}{7pt}
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Diagnostic} & \textbf{Context + predicted future} & \textbf{Context only} \\
\midrule
Presence F1 & 99.77\% & 99.58\% \\
Slot identity consistency & 70.29\% & 70.50\% \\
Slot ID switch rate & 4.05\% & 4.21\% \\
Target-object accuracy & 95.79\% & 94.02\% \\
Object-type accuracy & 92.86\% & 91.18\% \\
Color RGB MAE & 0.2244 & 0.2347 \\
Center MAE & 0.04541 & 0.04583 \\
Geometry MAE & 0.02851 & 0.02785 \\
Velocity MAE & 0.006295 & 0.005955 \\
\bottomrule
\end{tabular}
\end{table*}


==> Table/physion_future_semantics.tex <==
\begin{table}[t]
\centering
\caption{Effect of predicted-future evidence on present-state decoding.}
\label{tab:physion-future-semantics}
\small
\renewcommand{\arraystretch}{1.05}
\begin{tabularx}{0.70\linewidth}{@{}Lcc@{}}
\toprule\toprule
\textbf{Target} & \textbf{Context} & \textbf{Context + Future} \\
\midrule
Presence F1 & 99.58 & 99.77 \\
Target accuracy & 94.02 & 95.79 \\
Object type accuracy & 91.18 & 92.86 \\
\bottomrule\bottomrule
\end{tabularx}
\end{table}


==> Table/relation_information.tex <==
\begin{table}[t]
\centering
\caption{Relation-state readability at the pair--time level.}
\label{tab:relation-information}
\small
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Target} & \textbf{Metric} & \textbf{Score} \\
\midrule
Distance & $R^2$ & 0.5815 \\
Contact & AUROC & 0.9789 \\
Time-to-contact & $R^2$ & 0.5542 \\
\bottomrule
\end{tabular}
\end{table}


==> Table/relation_intervention.tex <==
\begin{table*}[t]
\centering
\caption{Relation-instance interventions on 372 valid object pairs.}
\label{tab:relation-intervention}
\scriptsize
\setlength{\tabcolsep}{2.6pt}
\begin{tabularx}{\textwidth}{@{}lYYYYYYY@{}}
\toprule
 & \multicolumn{3}{c}{\textbf{Entity / Dynamic}} & \multicolumn{3}{c}{\textbf{Relation}} & \textbf{Task} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
\textbf{Condition} & \makecell{Pres.\\AUC} & \makecell{Ext.\\MAE} & \makecell{Speed\\MAE} & \makecell{Pair dist.\\MAE} & \makecell{Contact\\AUC} & \makecell{TTC\\MAE} & \makecell{OCP\\AUC} \\
\midrule
Baseline & 0.9261 & 0.0307 & 0.0678 & 0.0196 & \best{0.9633} & 0.1306 & 0.6995 \\
Contact-pair mask & 0.9194 & 0.0345 & 0.0735 & 0.0225 & 0.9488 & 0.1376 & 0.6518 \\
Non-contact-pair mask & 0.9315 & 0.0354 & 0.0754 & 0.0208 & 0.9518 & 0.1349 & 0.6175 \\
\bottomrule
\end{tabularx}
\end{table*}


==> Table/videomae_ek100_generalization.tex <==
\begin{table}[t]
\centering
\caption{VideoMAE~v2 EK100 direct-head baseline: train--validation gap.}
\label{tab:videomae-ek100-gap}
\scriptsize
\renewcommand{\arraystretch}{1.03}
\begin{tabularx}{0.70\linewidth}{@{}Lccc@{}}
\toprule\toprule
\textbf{Split} & \textbf{Verb Top-1} & \textbf{Noun Top-1} & \textbf{Action Top-1} \\
\midrule
Train & 96.70 & 96.68 & 92.92 \\
Probe validation & 59.54 & 46.37 & 35.96 \\
\bottomrule\bottomrule
\end{tabularx}
\end{table}

